How Problematic Writer-AI Interactions (Rather than Problematic AI) Hinder Writers' Idea Generation

Writing about a subject enriches writers' understanding of that subject. This cognitive benefit of writing -- known as constructive learning -- is essential to how students learn in various disciplines. However, does this benefit persist when students write with generative AI writing assistants? Prior research suggests the answer varies based on the type of AI, e.g., auto-complete systems tend to hinder ideation, while assistants that pose Socratic questions facilitate it. This paper adds an additional perspective. Through a case study, we demonstrate that the impact of genAI on students' idea development depends not only on the AI but also on the students and, crucially, their interactions in between. Students who proactively explored ideas gained new ideas from writing, regardless of whether they used auto-complete or Socratic AI assistants. Those who engaged in prolonged, mindless copyediting developed few ideas even with a Socratic AI. These findings suggest opportunities in designing AI writing assistants, not merely by creating more thought-provoking AI, but also by fostering more thought-provoking writer-AI interactions.

==> cutting_room_floor.tex <==
\section{Abstract}

\section{Intro}
% To date, little research has investigated this question. Instead, researchers who created novel AI assistants often found that these systems prompted writers to take on entirely new thought processes and strategies. However, they were unable to conclude whether these processes enhanced or hampered idea generation (Figure~\ref{fig:MessyFlow})~\cite{Rambler_JDZamfi_CHI24,StoryAssembler,Tankelevitch_CHI24_MegacognitiveGenAI}.

% Nevertheless, it remains unclear when and how these impacts occur during the writing process. Such a deeper, more mechanistic understanding, researchers may struggle to keep pace with the evaluation efforts, as a wide variety of writing assistance systems rapidly adopt newer genAI models, from GPT-3 to GPT-4 to DeepSeek.
% Relatedly, educators and policymakers may find it difficult to determine which research findings about genAI writing assistant's impact on student learning are still valid. 
% As a result, as novel genAI models kept popping up and new writing assistant designs kept popping up, it is unclear which of these findings still stand. Moreover, as researchers created many novel AI assistants and found these systems prompted writers to take on entirely new thought processes and strategies, there were unable to conclude whether these processes actually enhanced idea generation.
% Additionally, researchers also found that many novel AI assistants prompted writers to take on entirely new thought processes and strategies, but it remains unclear whether these processes actually enhanced idea generation (Figure~\ref{fig:MessyFlow})~\cite{Rambler_JDZamfi_CHI24,StoryAssembler,Tankelevitch_CHI24_MegacognitiveGenAI}.

\section{Method}

This approach deviates from the common approach where researchers build a genAI assistant and evaluate its impact on writers' thought processes.
First, whether writing with or without AI assistance, writers alternate among various cognitive and metacognitive activities ``\textit{in a seemingly haphazard fashion}” during writing~(Figure~\ref{fig:MessyFlow}), making it difficult to tease out AI's impact.
By contrasting writers' thought processes when they are either stimulated or hindered by AI suggestions, we could more effectively discern when and how AI suggestions impacted writers' idea generation.
% writers do not typically carry out cognitive and metacognitive activities in an orderly manner but “\textit{move from solving one problem to another in a seemingly haphazard fashion}”~\cite{quinlan2012coordinating,pea1987cognitive}.
% \placeholder{Rationale is the thought process of writers are haphazard (Figure~\ref{fig:MessyFlow}), contrasting the two can help us cut through the noise.}


Noteworthily, the pace of semantic expansion is by no means a perfect measure of writers' idea generation speed.
Albeit imperfect, it was useful for this study.
In this study, the primary method for understanding writers' idea generation processes was through their own recollections, which, while useful, are highly subjective. In this context, semantic expansion offers a valuable complementary perspective; one based not on memory, but on the actual texts the writers produced moment by moment.
The findings we present in this paper are confirmed by both qualitative and quantitative data.

\section{Key interactions}
When participants passively relied on AI suggestions, one problematic AI suggestion could cause (sometimes unrecoverable) disruption to their writing processes.
For P4, the AI assistant's failure to generate a conclusion for his writing resulted in a final article with no conclusion.
